Learning Read-Once Determinants and the Principal Minor Assignment Problem

A symbolic determinant under rank-one restriction computes a polynomial of the form $\det(A_0+A_1y_1+\ldots+A_ny_n)$, where $A_0,A_1,\ldots,A_n$ are square matrices over a field $\mathbb{F}$ and $rank(A_i)=1$ for each $i\in[n]$. This class of polynomials has been studied extensively, since the work of Edmonds (1967), in the context of linear matroids, matching, matrix completion and polynomial identity testing. We study the following learning problem for this class: Given black-box access to an $n$-variate polynomial $f=\det(A_0+A_1y_1+ \ldots+A_ny_n)$, where $A_0,A_1,\ldots,A_n$ are unknown square matrices over $\mathbb{F}$ and rank$(A_i)=1$ for each $i\in[n]$, find a square matrix $B_0$ and rank-one square matrices $B_1,\ldots,B_n$ over $\mathbb{F}$ such that $f=\det(B_0+B_1y_1+\ldots+B_ny_n)$. In this work, we give a randomized poly(n) time algorithm to solve this problem. As the above-mentioned class is known to be equivalent to the class of read-once determinants (RODs), we will refer to the problem as learning RODs. The algorithm for learning RODs is obtained by connecting with a well-known open problem in linear algebra, namely the Principal Minor Assignment Problem (PMAP), which asks to find (if possible) a matrix having prescribed principal minors. PMAP has also been studied in machine learning to learn the kernel matrix of a determinantal point process. Here, we study a natural black-box version of PMAP: Given black-box access to an $n$-variate polynomial $f = \det(A + Y)$, where $A \in \mathbb{F}^{n \times n}$ is unknown and $Y = diag(y_1,\ldots,y_n)$, find a $B\in\mathbb{F}^{n\times n}$ such that $f=det(B+Y)$. We show that black-box PMAP can be solved in randomized poly(n) time, and further, it is randomized polynomial-time equivalent to learning RODs. We resolve black-box PMAP by investigating a property of dense matrices that we call the rank-one extension property.

==> Counter-Example.tex <==
\section{Extending Roshan's Conuter Example to general $n$}

For any $k\in [n]$, let $\nsubset{k}$ denote the set $[n]-k$. Suppose that $A$ is an $n\times n$ matrix of the following form:
\begin{equation}
\label{eqn:counter-example-one}
A=
\begin{pmatrix}
1                &  1                & 1                & 1          & a_{15}      & a_{16} &\cdots & a_{1n}\\
% &&&&&&\\
2                &  1                & 1                & 1          & a_{25}      & a_{26} & \cdots  & a_{2n}\\
% &&&&&&\\
1                &  1                & 1                & 2          & a_{35}      & a_{36} & \cdots  & a_{3n}\\
% &&&&&&\\
1                &  1                & 1                & 1          & a_{45}      &  a_{46} & \cdots  & a_{4n}\\
% &&&&&&\\
a_{15}           &  a_{25}           & a_{35}           & a_{45}     & 1           & a_{56} & \cdots  & a_{5n}\\
% &&&&&&\\
a_{16}           &  a_{26}           & a_{36}           & a_{46}     & a_{56}      & 1 & \cdots  & a_{6n}\\
% &&&&&&\\
\vdots           &  \vdots           & \vdots           & \vdots     &\vdots       &\ddots  & \vdots\\
% &&&&&&\\
a_{1n}           &  a_{2n}           & a_{3n}           & a_{4n}     & a_{5n}      & a_{6n} & \cdots & 1\\
\end{pmatrix}
\end{equation}
Now we show the following lemma.
\begin{claim}
\label{clm:conuter-example-tool}
Let $A$ be an $n\times n$ matrix over a field $\F$ with nonzero off-diagonal entries, and assume that$A$ is of the form given in~\cref{eqn:counter-example-one}. Suppose that $A$ has no cut $X$ such that $\{1,2\}\subseteq X$ and $\{3,4\}\subseteq \comp{X}$. Let $B$ is another $n\times n$ matrix such that 
\begin{equation}
\label{eqn:counter-example-two}
B[i,j]=A[i,j]\ \forall\, (i,j)\notin\{(1,2), (2,1)\},\ \ \   B[1,2]=A[2,1]=2, \text{ and } B[2,1]=A[1,2]=1
\end{equation}
Then, $\kPME{A}{B}{4}$, but $A\nPME B$.
\end{claim}
\begin{proof}
Observe that $A[\nsubset{j}]=B[\nsubset{j}]$ for $j=1,2$, and $A[\nsubset{j}]=B[\nsubset{j}]^T$ for $j=3,4$. Moreover, $B[\{1,2,3,4\}]=\tw\left(A, \{3,4\}\right)$. Thus, $\kPME{A}{B}{4}$, and $$\{1,2\}\subseteq \calD_1(A,B)\ \ \text{ and }\ \ \{3,4\}\subseteq \calD_2(A,B).$$ Since $A[\{1,2,3,4\}]\nDS B[\{1,2,3,4\}]$ and $A[\{1,2,3,4\}]\nDS B[\{1,2,3,4\}]^T$, $$ \calD_1(A,B)=\{1,2\}\ \ \text{ and }\ \ \calD_2(A,B)=\{3,4\}.$$ If $A\PME B$, then the above equation combined with~\cite[Theorem~2]{Loewy86} implies that $A$ has a cut $X$ such that $\{1,2\}\subseteq X$ and $\{3,4\}\subseteq \comp{X}$. This is a contradiction. Therefore, $A\nPME B$.
\end{proof}

\paragraph*{Explicit construction.} Using the above claim, an explicit construction of matrices $A$ and $B$ such that $\kPME{A}{B}{4}$ but $A\nPME B$ given below: Let $a\in \F$ such that $a\neq 0,1$. Then, 

\begin{equation}
\label{eqn:counter-example-three}
A=
\begin{pmatrix}
1                &  1                & 1                & 1          & a^{6}  & a^7      & \cdots & a^{1+n}\\
% &&&&&&\\
2                &  1                & 1                & 1          & a^{7}  & a^8     & \cdots  & a^{2+n}\\
% &&&&&&\\
1                &  1                & 1                & 2          & a^{8}  & a^9    & \cdots  & a^{3+n}\\
% &&&&&&\\
1                &  1                & 1                & 1          & a^{9}  & a^{10}    & \cdots  & a^{4+n}\\
% &&&&&&\\
a^{6}            &  a^{7}            & a^{8}            & a^{9}      & 1      & a^{11}    & \cdots  & a^{5+n}\\
% &&&&&&\\
a^{7}            &  a^{8}            & a^{9}            & a^{10}      & a^{11}      & 1    & \cdots  & a^{6+n}\\
% &&&&&&\\
\vdots           &  \vdots           & \vdots           & \vdots     &\vdots   & \vdots  &\ddots  & \vdots\\
% &&&&&&\\
a^{1+n}          &  a^{2+n}          & a^{3+n}          & a^{4+n}    & a^{5+n} & a^{6+n}   & \cdots & 1\\
\end{pmatrix},
\end{equation}
and $B$ is defined accoding to~\cref{eqn:counter-example-two}. 

Let $X\subseteq [n]$ such that $\{1,2\}\subseteq X$ and $\{3,4\}\subseteq [n]$. Since $n\geq 5$, there exists a $k\in[n]\setminus \{1,2,3,4\}$ such that either $k\in X$ or $k\in \comp{X}$. First, assume that $k\in \comp{X}$. Then, consider the submatrix $A[\{1,2\}, \{3,k\}]$. Since $\rank A[\{1,2\}, \{3,k\}]=2$, it follows that $X$ is not a cut. Next, suppose that $k\in X$. Then, $\rank A[\{1,k\}, \{3,4\}]=2$, which again implies that $X$ is not a cut of $A$. Thus, $A$ does not have any cut $X$ such that $\{1,2\}\subseteq X$ and $\{3,4\}\subseteq [n]$.  As explained in the proof of~\cref{clm:conuter-example-tool}, $\calD_1(A,B)=\{1,2\}$ and $\calD_2(A,B)=\{3,4\}$. Therefore, $A\nPME B$. However, since all the corresponding principal minors of size at most $4$ agree. Furthermore,  observe that $\rank A[\{1,2\}, \{3,4\}]=1$ but there does not exist $X\subseteq A$ with $1,2\in X$, $3,4\in \comp{X}$ and $\rank A[X, \comp{X}]=1$. Therefore, $A$ does not satisfy property $\prop$. 


Next, we present another construction of an $n\times n$ matrix $A$ of the form~\cref{eqn:counter-example-one} that satisfies the following properties:
\begin{enumerate}
\item for any matrix $B$ defined as per~\cref{eqn:counter-example-two}, we have $\kPME{A}{B}{4}$ but $A\nPME B$.
\item  The matrix $A$ does not satisfy property~$\prop$. Note that $\rank A[\{1,2\}, \{3,4\}] = 1$. However, the construction will imply that there does not exist a subset $X \subseteq [n]$ such that $1,2 \in X$, $3,4 \in \comp{X}$, and $\rank A[X, \comp{X}] = 1$. Furthermore, for every $k \in {5,6,7,\ldots, n}$, the principal submatrix $A[\nsubset{k}]$ admits a cut $X$ with $1,2 \in X$ and $3,4 \in \nsubset{k} \setminus X$, but such a set $X$ does not satisfy the conclusion of~\cref{lem:lift-of-cut}.
\end{enumerate}

In the second construction, we define the matrix $A$ as follows:
\[
A=
\begin{pmatrix}
1       &  1      & 1       & 1       & 1       & 1      & 1      & \cdots & 1       & \textcolor{red}{2}\\
% &&&&&&\\
2      &  1      & 1       & 1       & 1       & 1      & 1      & \cdots  & 1      & 1\\
% &&&&&&\\
1       &  1      & 1       & 2     & 1       & 1      & 1      & \cdots  & 1      & 1\\
% &&&&&&\\
1       &  1      & 1       & 1       & \textcolor{red}{2}       & 1      & 1      & \cdots  & 1      & 1\\
% &&&&&&\\
1       &  1      &  1      & \textcolor{red}{2}      & 1       & \textcolor{red}{2}      & 1      & \cdots  & 1      & 1\\
% &&&&&&\\
1       &  1      &  1      & 1       & \textcolor{red}{2}      & 1      & \textcolor{red}{2}     & \cdots  & 1      & 1\\
% &&&&&&\\
1       &  1      &  1      & 1       & 1       & \textcolor{red}{2}     & 1      & \cdots  & 1      & 1\\
% &&&&&&\\
\vdots  &  \vdots & \vdots  & \vdots  &\vdots   &\vdots  & \vdots & \cdots  & \vdots & \vdots\\
% &&&&&&\\
1     &  1      & 1       & 1       & 1       & 1      & 1      & \cdots  & 1      & \textcolor{red}{2}\\
% &&&&&&\\
\textcolor{red}{2}       &  1      & 1       & 1       & 1       & 1      & 1      & \cdots  & \textcolor{red}{2}     & 1\\
\end{pmatrix},
\]
that is,
\begin{enumerate}
\item $A[\{1,2,3,4\}]$ is defined as in mentioned in~\cref{eqn:counter-example-one}
\item For all $i\in\{5,6,7,\ldots, n\}$, $A[i-1, i]=A[i, i-1]=2$, and additionally  $A[1,n]=A[n,1]=2$
\item All the remaining remaining entries are 1.
\end{enumerate}
Let $k\in\{5,6,7, \ldots, n\}$, and $X=\{1,2,k+1, k+2, \ldots, n\}$ and $\comp{X}=\nsubset{k}\setminus X$, that is $\comp{X}=\{3,4,5, 6, \ldots k-1\}$. Observe that $X$ is a cut of the matrix $A[\nsubset{k}]$. 

Now, assume that $X\subseteq [n]$ such that $\{1,2\}\subseteq X$ and $\{3,4\}\subseteq \comp{X}$. Since $\rank A[\{1,2\}, \{3, n\}]=2$, in order for $X$ to be cut of $A$, it must include $n$. Continuing this reasoning inductively, we can show that $\{4,5,6,\ldots, n\}\subseteq X$, which contradicts the assumption $4\in \comp{X}$. Therefore, no such subset $X$ is a cut of $A$. 


These constructions demonstrate that property $\prop$ is necessary for concluding that $\kPME{A}{B}{4}$ implies $A\PME B$.
